AutoCAT: Reinforcement Learning for Automated Exploration of Cache-Timing Attacks

The aggressive performance optimizations in modern microprocessors can result in security vulnerabilities. For example, timing-based attacks in processor caches can steal secret keys or break randomization. So far, finding cache-timing vulnerabilities is mostly performed by human experts, which is inefficient and laborious. There is a need for automatic tools that can explore vulnerabilities given that unreported vulnerabilities leave the systems at risk. In this paper, we propose AutoCAT, an automated exploration framework that finds cache timing-channel attack sequences using reinforcement learning (RL). Specifically, AutoCAT formulates the cache timing-channel attack as a guessing game between an attack program and a victim program holding a secret. This guessing game can thus be solved via modern deep RL techniques. AutoCAT can explore attacks in various cache configurations without knowing design details and under different attack and victim program configurations. AutoCAT can also find attacks to bypass certain detection and defense mechanisms. In particular, AutoCAT discovered StealthyStreamline, a new attack that is able to bypass performance counter-based detection and has up to a 71% higher information leakage rate than the state-of-the-art LRU-based attacks on real processors. AutoCAT is the first of its kind in using RL for crafting microarchitectural timing-channel attack sequences and can accelerate cache timing-channel exploration for secure microprocessor designs.

==> FSM_old.tex <==

\subsection{Rationale for Using Reinforcement Learning in the Cache Guessing Game}
\label{sec:FSM_formulation}
%\vspace{-0.1in}

\hl{In this section, we discuss how a cache set can be represented as an FSM, 
and why RL is a good fit for the cache guessing game
given the RL method is known to be able to solve an MDP with an FSM.} 
As cache-timing attacks exploit the internal states of a cache, \hl{
the cache guessing game can be seen as an MDP that optimizes the correct guessing rate. 
All digital circuits including caches can be seen as FSMs.}


\hl{Note that we discuss an example FSM formation for the cache guessing game here mainly to show
that this problem setting matches the RL method in theory and 
provide a rational for using RL in the cache guessing game. 
In practice, however, RL method does not require the knowledge of FSM formulation, and the RL model in} {\acronym} \hl{directly interfaces
with a black box cache model to solve the cache guessing game. 
} 


\hl{To show the theoretical foundation, here we} consider a toy cache example with only one cache block and two cache lines 0 and 1. 
This simple cache can be represented by a FSM $\mathcal{M}=(\mathcal{S}, \mathcal{A}, \mathcal{P}\}$ where $\mathcal{S}=\{s_0, s_1\}$ contains the all cache states representing which addr (0 or 1) is in the cache, $\mathcal{A}=\{a_0, a_1\}$ contains  actions that access address 0/1, and $\mathcal{P}$ has the transition rules, shown as the arrows in Figure~\ref{fig:mdp}.

% why are they difficult to design

%Without deep understanding of the cache structure, it is hard to discover and design new cache-timing channel attacks.

%% how to represent a cache state to FSM


\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{figure/mdp}
\vspace{-6pt}
\caption{FSM of the cache guessing game for an example one-block cache with only two cache lines. [hit/miss] indicates the observation during a transition.
}
\label{fig:mdp}
\vspace{-12pt}
\end{figure}

%Currently we assume all state transitions $\mathcal{A}=\{a_0, a_1\}$ caused by memory access are the attacker's access.
%We can build on this FSM to introduce the concept of victim. 
We can formulate the cache guessing game based on the FSM of the cache with the additional state transitions for the victim's accesses ($a_\text{v}$) and the attacker's guess ($a_\text{g0}$ or $a_\text{g1}$).
In a typical cache timing-channel threat model, the victim holds a secret address $addr_{secret}$ which is unknown to the attacker. 
For example, if the secret address is either address 0 or address 1, then we can add an action $a_\text{v}$ to $\mathcal{A}$ to represent an access to the secret address.
%\footnote{We can optionally configure whether we allow the victim to make no access, which also leaks information and use a specific address to represent it.}
%, and we can use a default $addr_{secret\_e}$ value to represent this scenario.}
As the attacker does not know the secret address, this action may lead to $s_0$ or $s_1$ depending on the secret as shown in Figure~\ref{fig:mdp}. 
We add two actions $a_\text{g0}$ and $a_\text{g1}$ to $\mathcal{A}$ indicating that the attacker makes a guess that the secret address is 0 or 1. 
We also add two additional states $s_\text{c}$ and $s_\text{w}$ to $\mathcal{S}$ to represent the guess is correct or wrong.
The transition $\mathcal{P}$ depends on $addr_{secret}$.

A successful attack sequence that can be represented as a path starting from $s_0$ or $s_1$ and ends in $s_c$ in Figure~\ref{fig:mdp}, whereas a failed attack sequence ends in $s_w$. 
The goal is to find as many successful attacks as possible. 
For example, assume we start with $s_0$, and we want to end in $s_c$. We can reach $s_c$ by taking action $a_{g0}$ or $a_{g1}$ depending on the value of $addr_{secret}$, which is unknown to the attacker. However, $addr_{secret}$ can be inferred by the state after $a_v$. For example, if after $a_v$ it ends in $s_1$, then $addr_{secret}$ must be 1. To infer the current state, we can do $a_1$ and observe the hit/miss response. Thus, if ${addr}_{secret}=1$, a successful attack \hl{sequence} can be: $s_0 \rightarrow a_v \rightarrow s_1 \rightarrow a_1 \text{(hit)} \rightarrow s_1\rightarrow a_{g1} \rightarrow s_c$. Similarly, if ${addr}_{secret}=0$, a successful attack \hl{sequence} can be: $s_0 \rightarrow a_v \rightarrow s_0 \rightarrow a_1 \text{(miss)}\rightarrow s_1\rightarrow a_{g0} \rightarrow s_c$.


%% Questions to Yuandong, Xiaomeng, Amy:
%% is this still called MDP? The p is either 0 or 1 (thus determinstic, but unknown, and changes from episode to episode, is it still called MDP or is it called something else? Is there a terminology for this? I thought for MDP, the p is a deterministic value in between 0 or 1 that does not change.

%% Hi Mulong, 

%If p can change from episode to episode, then we can treat these multiple episodes as one big episode within a new larger MDP, in which the states are copied with some modifications, so that they reflect the changes of the transition structure. 

%Best,
%Yuandong

%This formulates into an Markov decision process (MDP).


%% how traditionally that can be done
%% FSM traversal, enumeration

%Traditionally, with this MDP formulation we can use (linear/convex) optimization \cite{FIXME} to find an optimal solution. 
%However, practically, these are several challenges in using an optimization-based approaches.
This example shows that for all possible values of $addr_{secret}$ and initial states if we can enumerate all paths that lead to $s_c$, we can find all possible attacks. However, this search approach does not work in practice for the following reasons:

%\begin{enumerate}
%  \setlength{\itemsep}{0pt}
%  \setlength{\parskip}{0pt}
%  \setlength{\parsep}{0pt}
    %% 1. replacement policy, others not known (unknown FSM)
%    \item It is difficult to know the exact representations of the FSM because the detailed microarchitectural operations are often kept as proprietary confidential know how by chip designers. Reverse engineering effort can be onerous and only reveal limited information~\cite{abel2014reverse,vila2020cachequery}.
    %% even if the FSM is known
%    \item The state is not fully visible to the attacker because the state depends on other processes' cache entries.
    %% 2. sub-FSM, composition of multiple FSM increases complexity
%    \item There are multiple FSMs including a cache FSM, a replacement-state FSM \cite{perez2011functional}, cache directory FSM \cite{yan2019attack}, \hl{cache prefetcher}~\cite{wang2019papp,chen2021leaking}, etc. The composition of these FSMs multiples the number of states and transitions, making optimization-based methods intractable. 
    % if the states gets involved with the pipeline, this makes it even harder
    %% 3. non-determinstic transitions
%    \item Microarchitectural operations can be pseudo-random such as random replacement algorithms, meaning the transitions inside the FSM are not  entirely predictable.%, which complicates the optimizations.
%\end{enumerate}
%\hl{Due to these difficulties, directly using a search approach to enumerate all possible paths and find successful attacks is not practical. 
%Instead, we use RL that does not need the knowledge of the full FSM and does not need full observation of the state space.}
%% problems
%\hl{Applying RL to the cache-timing attack, we only need to define the rewards $\mathcal{R}$ and a black box cache~model.} 
%Since we want the policy to find successful attacks that end in $s_c$, we assign positive reward to that state. Since we do not want the policy to find unsuccessful attacks that end in $s_w$, we assign negative reward to that state. Also, as we do not want the policy to take unnecessary steps, we can also assign a relatively small negative reward for each step. 
%{\bf $\gamma$ is usually tuned during the RL training processes.}






% how MDP and finite state machine (FSM) are related? cache is controlled by FSM. 
% 
% RL = solving (partial observable) MDP =   

%Traditionally there are many timing-based side channel attacks.

%$addr_{secret}$
